Developing Story: Case Studies of Generative AI's Use in Journalism

Journalists are among the many users of large language models (LLMs). To better understand the journalist-AI interactions, we conduct a study of LLM usage by two news agencies through browsing the WildChat dataset, identifying candidate interactions, and verifying them by matching to online published articles. Our analysis uncovers instances where journalists provide sensitive material such as confidential correspondence with sources or articles from other agencies to the LLM as stimuli and prompt it to generate articles, and publish these machine-generated articles with limited intervention (median output-publication ROUGE-L of 0.62). Based on our findings, we call for further research into what constitutes responsible use of AI, and the establishment of clear guidelines and best practices on using LLMs in a journalistic context.

==> latex/ethicalConsiderations.tex <==
This study is motivated by a recognition that generative AI capabilities are rapidly evolving and their potential impacts on journalism call for thoughtful, thorough research.
%
Our goal is to provide insights that can help shape guidelines and policies governing the responsible use of AI in this domain. 

We hypothesize that Agencies~A and~B are not unique cases of news organizations using generative AI, but rather examples of a broader phenomenon that happen to be present in the WildChat dataset.
%
Furthermore, the intent of this work is not to ``call out'' specific agencies or individual users, but to investigate and better understand the actual use of generative AI in journalism. 
%
Accordingly, we have anonymized the identities of the agencies in this paper.

Although we anonymize the agencies' names and censor identifying information, we provide metadata and verbatim text that could be used to identify them. 
%
We include this information for scientific rigor and thoroughness as well as recognize that, even without it, others could independently identify the news agencies through WildChat.
%
However, we do not encourage or condone the use of this data beyond our stated purpose of understanding AI usage in journalism. 
%
Our intent is to advance knowledge, not target or harm any individuals or organizations. 
